On Fair Ordering and Differential Privacy

In blockchain systems, fair transaction ordering is crucial for a trusted and regulation-compliant economic ecosystem. Unlike traditional State Machine Replication (SMR) systems, which focus solely on liveness and safety, blockchain systems also require a fairness property. This paper examines these properties and aims to eliminate algorithmic bias in transaction ordering services. We build on the notion of equal opportunity. We characterize transactions in terms of relevant and irrelevant features, requiring that the order be determined solely by the relevant ones. Specifically, transactions with identical relevant features should have an equal chance of being ordered before one another. We extend this framework to define a property where the greater the distance in relevant features between transactions, the higher the probability of prioritizing one over the other. We reveal a surprising link between equal opportunity in SMR and Differential Privacy (DP), showing that any DP mechanism can be used to ensure fairness in SMR. This connection not only enhances our understanding of the interplay between privacy and fairness in distributed computing but also opens up new opportunities for designing fair distributed protocols using well-established DP techniques.

==> dp_prev_writeup.tex <==

\section{Old DP write-up. }
As in Pompe, we model replica preferences with ordering indicators. However, we dive deeper to understand what affects those indicators. These indicators are not assigned in a void, but they are influenced not only by the command itself and its metadata but also by external, irrelevant information. A simple example that will accompany us throughout the paper is network delays. That is, a node may prefer one command over the other because of different delays on the route from the original clients.


To this end, we define the ordering indicator as a function \emph{score}$:\mathcal{C}\rightarrow \mathcal{O}$ that maps a command $c$ to an indicator $o$. 
The inputs of \emph{score} are the relevant features $\emph{metadata}$ and irrelevant features $\eta_{irr}$ associated with a specific command. 
To comply with existing deployed systems, we focus in this paper on numerical scores, where \emph{score} is computed by implicitly summing relevant and irrelevant features. 
In the case of network delays-- a relevant piece of information is the time of invocation by the client, whereas the time frame it took the command to be sent over the network towards different replicas is irrelevant. However, unconsciously, any correct replica sums these two values together when assigning a suggested timestamp. E.g., a client located in Brazil issues a request at $5:00$ PM. Since one of the replicas is located in India, it may receive it with a 2-minute delay, assigning $5:02$ PM as the indicator.
Note that this is not a Byzantine behavior, a correct replica is doomed to naively make this sum, as it cannot distinguish the relevant and irrelevant information. Also note that in order to prevent Byzantine clients from spreading misleading information, we cannot rely on a client to provide a correct time of invocation in this example.


Another example of an additive score function is in the context of transaction fees, where replicas may want to set their preferences according to the amount of revenue they make by setting one command before the other. In this case, relevant information would be the fees corresponding to block transactions. On the other hand, any kickbacks exposed by clients are irrelevant and should be masked when aiming for fair ordering. More on that example in~\ref{sec:DP_for_miners_fees}.


Looking closely, we can also divide the irrelevant features into two categories: irrelevant features that are implicitly taken into consideration by the protocol and bias the ordering indicators, and some irrelevant information that is completely orthogonal to the system design. This information varies in different protocols but can include for example the content of the command, the IP of the client, etc.
Unfortunately, when building a Byzantine fault-tolerant system we can never be sure about the way Byzantine replicas assign the ordering indicators. 
Specifically, they might take into consideration information that is overlooked by correct replicas, deepening the bias of their indicators. To model their arbitrary behavior, we add an extra noise $\eta_b$ that captures Byzantine bias (this noise can be both positive and negative). For correct replicas, it holds that $\eta_b=0$. 


Formally, 
\begin{equation*}
    \emph{score}(c)=\text{metadata}+\eta_{irr}+\eta_b
\end{equation*}
where metadata holds the relevant information, $\eta_{irr}$ is the noise from irrelevant features that are implicitly biasing the indicator (in opposition to orthogonal irrelevant features), and $\eta_b$ is any noise further exposed by Byzantine behavior. 

Our objective in this paper is to overcome inherent noise originating in the environment as well as being resilient to intentional noise that may be exposed by Byzantine replicas.
In practice, we cannot distinguish between the two different types of noises $\eta_{irr}$ and $\eta_b$. Thus, we replace the two with arbitrary noise $\eta=\eta_{irr}+\eta_b$ which we handle de facto. From hereon we examine the function 
$\emph{score}(c)=\text{metadata}+\eta$.
For ease of explanations, we will denote by $c.\emph{metadata}$ and $c.\eta_i$ the metadata and noise components that were used to calculate command $c$'s score at replica $i$. Note that $c.\emph{metadata}$ is missing a subscript for the process. That is because for any command $c$ by definition $\emph{metadata}$ is the same at all replicas.

% captured in the system as a noise.
% We can also use sigmas here, I don't think we need though

% since we assume bound on irrelevant information
% Our objective in this paper is overcoming inherent noise originating in the environment as well as being resilient to intentional noise that may be exposed by Byzantine replicas.

The context in which we use these ordering indicators are for ordering commands as part of an ordering mechanism.
A \emph{Ordering Mechanism} $\mathrm{Ord}:\mathcal{C}\times \mathcal{O}^n\rightarrow \mathcal{O}$ is an algorithm that given a command and a set of ordering indicators for that command, returns a single ordering indicator. The resulting indicator for each command determines its place in the total order of commands.
In our case, replicas use \emph{score} to express their ordering preferences, taken as an input to $\mathrm{Ord}$.

\subsection{$\epsilon$-Ordering Equality}


Understanding the low-level structure of ordering indicators allow us to examine ordering fairness in higher resolution than what was previously done. Intuitively, a ``fair'' ordering mechanism should give heavy weight to the metadata component of \emph{score}, and ideally ignore the rest. In other words, we aim at increasing the signal of metadata and conceal $\eta$. 

Let $c,c'$ be two commands issued by clients.
% , and let $i,j$ be any two replicas.
% Let $\langle \emph{metadata},\eta \rangle$ and $\langle \emph{metadata}',\eta' \rangle$ be the components of their \emph{score} outputs by any two replicas, accordingly.
We say that $c$ and $c'$ are \emph{adjacent}, denoted as $c \sim c'$, if and only if their relevant features are the same, i.e., $c.\emph{metadata}=c'.\emph{metadata}'$. Under these notations, a fair ordering will not be able to differentiate any adjacent commands $c\sim c'$ and a fair protocol will give them equal opportunity in terms of which one gets to be served first. We capture this desired behavior in a property called \emph{$\epsilon$-Ordering Equality}.


% \shir{this is a property of ordering algorithm, the definition of such algorithm should be added here}

Formally,


\begin{definition}[$\epsilon$-Ordering Equality]

    $\mathrm{Ord}$ provides $\epsilon$-Ordering Equality if for any two commands $c\sim c'$ it holds that
\begin{equation*}
    Pr[c\prec c'] \le e^{\epsilon} Pr[c'\prec c].
\end{equation*}
    
\end{definition}





As one might suspect, it is impossible to handle any amount of noise that is being added to the meaningful information when computing \emph{score}.
That is, there are cases where it impossible to satisfy $\epsilon$-Ordering Equality. In a nutshell, when the noise in the system $\eta$ is too high, it becomes impossible to distinguish it from the metadata signal. Once again, this can happen due to amplification of irrelevant information and/or uncontrolled Byzantine behavior.
Therefore, we define a threshold $\lambda$ on the amount of noise we can handle. Formally, for two commands $c,c'$ and any two replicas $i,j$ we use norm L1 to reason about their difference in noise.
% We denote by  $\lVert c-c' \rVert_1$ the subtraction of their corresponding noises components $\eta, \eta'$, as implicitly expressed in \emph{score}. \shir{TODO: denote the noise function here already, and use it in the assumption}
% \footnote{This notation is only useful for adjacent commands.}
% Using this notation, 
We make the following assumption:

\begin{assumption}
\label{assumption:bound_on_noise}
There exists a system parameter $\lambda$ s.t.
            \[\lambda =\max_{c,c',i,j} \lVert c.\eta_i-c'.\eta_j \rVert_1 \]
where $c\sim c'$.
\end{assumption}

When instantiated with the ``right'' $\lambda$, $\epsilon$-Ordering Equality can be satisfied.


\shir{this will later relate to the l-sensitivity}



\shir{minor: similar to SNR?}


\shir{possible place for a bonus formal lower bound, if we have time later}



% is supposed to be plausible with respect to the metadata component, and resistant to biasing noise. That is, the order should be affected by the metadta component 



% Eventually, we are trying to provide the following fairness property:







% Consider any two commands $X, X' \in \mathcal{X}^n$, which differ in exactly one entry. We call these neighbouring datasets, and sometimes denote this by $X \sim X'$. 




\subsection{$\epsilon$-Differential Privacy}

We suspect that some readers may experience a  slight feeling of deja vu by this point. Indeed, our definitions resemble ones from a completely different realm-- differential privacy. This is not just an innocent mistake.
Our key insight in this work is laying down the connection between removing bias for ordering fairness and differential privacy.
Differential privacy is a way to quantify how much information is leaked by an algorithm.
It quantifies how much the algorithm's output changes as the input of the algorithm is tweaked.
If the algorithm's outputs do not change significantly, then the amount of information contained in the output about the input is limited.
Indeed, this is exactly what we are trying to do.
While we are not concerned with hiding the noise $\eta$ at all, we wish to guarantee that the value of $\eta$ does not affect the final ordering-- precisely the notion that differential privacy captures.
For completeness, we provide here the definition for Differential privacy.






Suppose we have an algorithm $M : \mathcal{X}^n \rightarrow \mathcal{Y}$. Consider any two datasets $X, X' \in \mathcal{X}^n$, which differ in exactly one entry. We call these neighbouring datasets, and sometimes denote this by $X \sim X'$. 

\begin{definition}[$\epsilon$-Differential Privacy]
$M$ is \textit{$\epsilon$ differentially private} if, for all neighbouring $X, X'$, and all $T \subseteq \mathcal{Y}$, we have

\[ \text{Pr} [M(X) \in T] \leq e^{\epsilon} \text{Pr}[M(X') \in T] \]

where the randomness is over the choices made by M.

\end{definition}

Given this definition, we now want to know how to construct a $\epsilon$-differentially private algorithm.
While there are many specialized techniques to guarantee $\epsilon$-Differential privacy in particular scenarios, there is a simple general purpose technique that works for all numerical values called the \emph{Laplace mechanism}.

It works as follows. First, define the $\ell_1$-sensitivity of a function:

\begin{definition}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}$.
The $\ell_1$-sensitivity of $f$ is:

\[\Delta^{(f)} = \max_{X, X'} \left\Vert f(X) - f(X') \right\Vert_1\]

where $X$ and $X'$ are neighboring datasets.
    
\end{definition}

At a high level $\Delta^{(f)}$ quantifies how sensitive $f$ is to a single input naturally.
If $f$, for example, always outputs $1$ irrespective of the input, then the Laplace mechanism does not need to do anything to hide the inputs- $f$ does it already!
As its name suggests, the Laplace mechanism uses the Laplace distribution defined here:\shir{I'm not sure we'll need the definition of the distribution, hopefully we can prove without using it directly }

\begin{definition}
    The \emph{Laplace distribution} with a location parameter of $0$ and a scale parameter of $b$ has the following density:

    \[
    p(x) = \frac{1}{2b}\exp{\frac{-|x|}{b}}
    \]
\end{definition}

This is denoted by Laplace($b$). The Laplace mechanism is defined as follows:

\begin{definition}
\label{def:laplace}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}$.
The \emph{Laplace mechanism} is defined as

\[
M(X) = f(X) + Y
\]

where $Y$ is sampled from \emph{Laplace}($\frac{\Delta}{\epsilon}$).

\end{definition}

Prior work has shown that this definition produces a differentially private mechanism, which we state in a theorm here:

\begin{theorem}
\label{thm_laplace}
    The Laplace mechanism $M$ is $\epsilon$-differentially private.
\end{theorem}

\section{Equivalence}

\soumya{If I say it, it must eventually happen, right?}\shir{yes, but before the deadline :-) }
In this section, we will prove that an ordering mechanism $\mathrm{Ord}$ guarantees $\epsilon$-ordering equality if and only if it also guarantees $\epsilon$-differential privacy. \shir{we are only going to prove one side of the reduction, we can think later about the other side}

\shir{TODO: add text here explaining what we're about to do, and that we assume a single ordering indicator at this point. this indicator is going to be the output of $\mathrm{Ord}$. so basically it's going to be like a "gadget" on top of Ord- you're running ord- achieve an agreement on an indicator, then applying the gadget- get a final new indicator. Also- using this approach might be useful when proving that ordering linearizability, given that the basic Ord provides it (or not... anyhow- i think it's nice but we might need to modify the theorem below, the proof itself should remain almost the same)}


\begin{theorem}
\label{thm:equivalence}
    Let $f: \mathcal{C} \rightarrow \mathbb{R}$ be a function that for a given command $c$ returns the noise $\eta$.\footnote{I.e., $f(c)=c.\eta$.} If the Laplace mechanism is applied for $f$ with $\Delta=\lambda$, then $\mathrm{Ord}$ provides $\epsilon$-ordering equality.
\end{theorem}
\begin{proof}

    Let $c,c'$ be two commands such that $c\sim c'$.
    By Assumption~\ref{assumption:bound_on_noise}, there exists a bound $\lambda$ such that $\lambda$ is the $\ell_1$-sensitivity of $f$. By Theorem~\ref{thm_laplace}, $M(c)=f(c)+Y$
    is $\epsilon$-differentially private.
    That is, by definition,

    \[ \text{Pr} [M(c)\in T] \leq e^{\epsilon} \text{Pr}[M(c')\in T] \]

I.e.,

    \[ \text{Pr} [f(c)+Y\in T] \leq e^{\epsilon} \text{Pr}[f(c')+Y\in T] \]

Therefore, the probability of differentiating the different noises after applying the Laplace mechanism is arbitrarily small. By the definition of adjacent commands, it holds follows that:
    \[ \text{Pr} [\emph{score(c)}=s] \leq e^{\epsilon} \text{Pr}[\emph{score(c')}=s] \]

    \[ \text{Pr} [\emph{score(c')}=s] \leq e^{\epsilon} \text{Pr}[\emph{score(c)}=s] \]


Finally, since $\mathrm{Ord}$ order commands according to their ordering indicator, which is captured by \emph{score}:
\begin{equation*}
    Pr[c\prec c'] \le e^{\epsilon} Pr[c'\prec c]
\end{equation*}

    satisfying $\epsilon$-Ordering Equality.

\end{proof}

\[
    Pr[c\prec c'] \le e^{\epsilon} Pr[c'\prec c]
\]

\[
Pr[c\prec c'] = \sum(kPr(score(c) = s)Pr(score(c') = s'))
\]
\[
Pr[c'\prec c] = \sum(kPr(score(c') = s)Pr(score(c) = s'))
\]

\[
Pr[c\prec c'] = \sum(kPr(score(c) = s)Pr(score(c') = s')) \leq \sum(k e^{\epsilon}Pr(score(c') = s) e^{\epsilon}Pr(score(c) = s'))
\]
\[=e^{2\epsilon}\sum(kPr(score(c') = s)Pr(score(c) = s')) =e^{2\epsilon}Pr[c' \prec c]\]

% \shir{Of course the above proof is true for ordering mechanisms that indeed ordering according to the indicators- as would happen in a centralized system. this is not the case for us, and I lied at "Finally...". We need to tie it with the new protocol. but I cannot prove anything about it because I don't know what it does exactly...
\shir{Below are my guidelines for the proof, i used 1 and 2 in the proof above. there will be another theorem that states Algorithm pompe* provides OE, using this theorem, points 3 and 4 . Also- the writing of course will need more work}

guidelines for proof:
\begin{enumerate}
    \item f(x) is $\eta$. command$\rightarrow$ noise
    \item $M(x)=\eta+ laplace noise$
   \item  we cannot calculate $M(x)$ directly because we don't know f, but since score is additive, it is equivalent to adding the noise onto score
 \item    later we say we want laplace noise to be random so it is calculated together by all replicas
\end{enumerate}




% \begin{theorem}
%     Orderdering mechanism output the same order indicator at all correct replicas
%     these agreed indicators determines the total order
% \end{theorem}




Theorem~\ref{thm:equivalence} draws the line that connect $\epsilon$-ordering equality and differential privacy. However, it is still unclear how to take advantage of this connection in our setting. Specifically, two questions stand above all others. First, how does one access the function $f$ that associate a command with its noise? Intuitively, if we could isolate the noise then the path to fair ordering becomes trivial. To Overcome this obstacle we benefit from the fact that noise is added to the command by summing. Using this fact, adding the Laplace sample to the ordering indicator has the same affect as adding it directly to the noise (as can be hinted by Theorem~\ref{thm:equivalence} proof). That means that in fact we do not need to know $f$, but the ordering indicator themselves that are easily accessible. 
The second challenge is how to sample the Laplace variable in a distributed manner. While each correct replica can be trusted to provide a random sample, it is not clear what Byzantine replicas will sample. Moreover, we want all replicas to sample the same noise, so that they produce the same total order. These requirements somewhat resembles the ones required from a \emph{shared coin} primitive~\cite{}. The main difference is that unlike a shared coin, that is defined with respect to some success rate parameter, we ought to always return the same result at all correct replicas.
To this end, we present a new primitive \emph{shared randomizer}. Formally, 

\begin{definition}

A shared randomizer takes \shir{fill in} as an input and produce a random sample $s$, such that the following properties hold:
\begin{itemize}
    \item Agreement. correct replicas agree on output
    \item Randomness. output is random according to some distribution
    \item Termination. all correct replicas output a value
\end{itemize}

\end{definition}

In this chapter we assume the existence of a shared randomizer.
Section~\ref{sec:rendomizer} presents two different implementation of such a primitive.




\begin{theorem}
    Algorithm~\ref{pompoe*?} satisfies $\epsilon$-ordering equality.
\end{theorem}
\begin{proof}

    proof sketch:
    \begin{enumerate}
        \item by ord properties (that one may want to define...), ord returns the same indicator $o$ for command $c$ at all correct replicas
        \item  we fulfill assumption 1 with $\lambda=\delta$ (the network delay), because the system is synchronous, and any noise beyond the networks delay will be ignored (this bounds Byz. behavior)
        \item by shared randomizer, all correct replicas return with the same laplace sample
        \item adding noise to the shared $o$ is the same ass adding it to $f(c)$
        \item together with theorem 2 , we provide OE
    \end{enumerate}
\end{proof}
    

==> dp_stuff.tex <==
\section{Differential Privacy of Uniform Noise}
It is known\footnote{The proof is a little involved, but this paper is the least involved I found that works out this result (See Theorem 1 on page 5, set $\alpha = 0$): https://proceedings.mlr.press/v89/geng19a/geng19a.pdf} that uniform noise has $(0,\delta)$-differential privacy. $\epsilon = 0$ means that the mechanism is \say{perfectly} private (by differential privacy standards), but there is some probability $\delta$ that the privacy is worse. $(\epsilon, \delta)$-differential privacy is a relaxed definition of differential privacy that says a mechanism has $\epsilon$-differential privacy with probability $1 - \delta$ and worse with probability $\delta$. How much worse and what $\delta$ looks like depends on context.

\subsection{Bercow}
The question is how does $\delta$ appear in Bercow. Computing $\delta$ for uniform noise requires knowing the range of values the noise is being selected from and the query sensitivity (maximum difference of two query outputs). In Bercow terms, the range of values is $\Delta_{noise}$ and the query sensitivity is the upper bound of network latency $\Delta_{net}$. This yields that $$\delta = \frac{\Delta_{net}}{\Delta_{noise}}$$
There seems to be some connection between differential privacy and fairness in the context of Bercow. $\epsilon = 0$ seems to say that Bercow is \say{perfectly} fair but $\delta > 0$ says that Bercow is not \say{perfectly} fair with some probability.

\subsection{$\epsilon$-Ordering Equality}
We define $\epsilon$-Ordering Equality similarly to \textit{Differential Privacy Applied to Ordering Equality}: \[ Pr[c \prec c'] \leq e^{\epsilon}Pr[c' \prec c] + \delta \] with the key difference is adding a $\delta$ term, similar to how approximate differential privacy modifies differential privacy. We claim this definition is also the definition in \textit{Bercow} if $\epsilon = 0$. With $\epsilon = 0$, we have \[ Pr[c \prec c'] - Pr[c' \prec c] \leq \delta \] where $\delta$ here is equivalent to $\epsilon$ in \textit{Bercow}. Note that the $\delta$ found in section $2$ is not a tight upper bound. However, it is a close approximation that is much easier to write, and this was noted in the supplementary materials of the Bercow paper.


==> leftovers.tex <==

\subsection{Objectives}

In the rest of the paper we try to answer the following questions:
% We're interested in the following questions: (first two are Fred's, then added more)
\begin{enumerate}
    \item What policies are feasible? What are not?
    \item What are the clients' capabilities to disrupt the enforcement of a policy?
    \item What "protections" mechanism can we offer against the latter?
    \item How do the previous answers change in the presence of Byzantine?
    
\end{enumerate}




\section{The Importance of Time}

\shir{fred: in comment}
% stabilityi
% sMR tutorial
% ziplog declaration may be giving stability



Our first observation is that the requests' time of arrival is inherent in ordering for a policy to be valid, as implied by Non-Blocking and Monotonic Order.
This makes total sense-- the system cannot decide on the order of an unknown request. An exception for this case is the work of Ziplog, where requests are being ordered prior to their arrival, based on requests prediction in systems with high throughput clients where some a-prior knowledge is available. Their ordering however, does not provide our Monotonic Order property.

That being said, except for providing a lower bound for a request order, time of arrival is not necessarily used. For example, we can think about requests that holds, in addition to their data, a metadata that includes a desired deadline for the request to be executed. A policy that order requests base on their \say{time-to-live} (TTL) is also valid. That is true because none of the properties require that requests are immediately ordered\shir{according to the second non-blocking version}. In fact, there is no limit on the amount of time a request can spend in he pending set. This can be monitored with an additional utilization property, that puts an upper bound on the time a requests can remain unordered at the server. Another utilization property can be less restrictive, and demands hat if the pending set is not empty, some request has to be ordered\shir{this is the first non-blocking option}.









\subsection{\shir{NEW}}
I've been doing some research on how we can verify and correctly measure features:
\begin{enumerate}
    \item  It looks like we aim at something called "consistency check" that is part of data validation. nothing to do with this information, i could find sophisticated methods for doing that.
    
    \item I thought regarding time of issue being a relevant feature, and assuming a single server for now:  the server can assigned 3 trusted "measurers" , each one can record  the delay from the time stated by the client. like GPS, this gives estimation on clients location, so the servers fourth measurement can be cross validated.

    \item I think actually he story is something like this: perfect fairness is impossible for some features. Pompe 2 had recognized it already, hence the epsilon in the OE definition. we enhance it so that also similar relevant features has similar chances. this solves (1) clients are unable to accurately measure, (2) Byzantine clients try to manipulate measurements.

time of issue is an example for (1) -- although pompe2 doesn't declare these times, the recorded time at servers is not a ground truth of distance, and there are also external factors such as network contention, environmental factors etc.



txn fees is example for (2) -- byzantine clients will take minimal steps to reorder. i.e, if i offer 10 coins, they might offer 10.0001 coins. We want the system to be robust to those kind of attacks. If the byzantine decides to put 15 coins, sure we will prefer his txn, and that is fair. its a completely different "class" in the relevant features measurement.

we will use laplacian noise to implement that. not sure if we should call it dp

\item We do not pretend in this work to decide which features are relevant. This is a decision of the system designer.
\end{enumerate}

% As a first example, let us consider the first-come-first-served policy (FCFS). Following this policy, a server that receives a request immediately order it after all previously received requests. The reader can verify that FCFS is a valid policy. Indeed, FCFS is a favorably method for ordering requests in many deployed systems~\cite{add citations}. 




\section{Fair Policy}


there is an order relation between relevant features.



\begin{algorithm}
    \begin{algorithmic}[1]
    \State $O:$ sequence of the requests ordered
    \Statex
    \While{$P\neq \varnothing$}

        \State \textcolor{gray}{adjust\_features$(P)$} \Comment{will be used in section XX}

        \State $\textit{high\_priority}\gets \{r\in P | r.relevant = minimum\}$ \Comment{will write correctly later...}
        % \{r.\textit{relevant}\}$

        % \State $\textit{high\_priority}\gets \operatorname*{arg\,max}_{r\in P}
        % \{r.\textit{relevant}\}$

        \State $\textit{next\_r}\gets \textit{high\_priority}.\textit{pick\_one}()$\Comment{uniformly random pick from the set}
        \State $P\gets P\setminus\{\textit{next\_r}\}$
        \State $O.\textit{add(next\_r)}$
        
    \EndWhile

    
    % \algstore{policy}

    \end{algorithmic}
    \caption{Policy: code for server}
    \label{alg:BB_main}
\end{algorithm}

\begin{theorem}
    Algorithm 1 implements a fair policy.
\end{theorem}


  Proof  TBD: will not be in the main body


==> long_sections/abstract_long.tex <==

In blockchain systems, fair ordering of clients' transactions is crucial for establishing a trusted and regulation-compliant economic ecosystem. Unlike traditional State Machine Replication (SMR) systems, which only require liveness and safety properties, the new use case also requires a system to exhibit a fairness property.
This paper examines such properties and aims to eliminate algorithmic bias in an ordering service, usually implemented by SMR.

Our starting point is the recently proposed notion of equal opportunity. In this model, transactions are characterized by relevant and irrelevant features, and the requirement is that the order is determined solely by the relevant features. Transactions with the same relevant features should have the same chances of being ordered before one another. We adopt this framework but generalize the idea to design a property that also captures the desired behavior for transactions with different relevant features.
In a nutshell, our definition requires that the greater the distance between transactions, according to their variance in the relevant features, the higher the probability that we prioritize one over the other.

We present a surprising connection between equal opportunity, defined in the context of SMR, and Differential Privacy (DP). We demonstrate that any DP mechanism can be utilized to ensure fairness in SMR. This connection not only enriches our understanding of the interplay between privacy and fairness in distributed computing but also opens up new possibilities for designing fair distributed protocols using well-established DP techniques.

==> long_sections/applications_old.tex <==


\subsection{Differential Privacy on Miner Fees}
% \label{sec:DP_for_miners_fees}

Another scenario where this technique can be applied is to construct bribery-proof consensus mechanisms.
In many blockchain systems, commands are first gossipped to all replicas before they are sequenced.
Upon sequencing, the leader typically receives a protocol defined fee for their efforts and a per-command fee that is paid by the clients to the leader in order to indicate the importance of the command.
This way, a command that pays Starbucks for a coffee is given lower priority than a command that is transferring funds to buy a house.
However, there are cases where the leader may receive out of band side payments from the client to order their commands preferentially.
These side payments are typically used to maliciously reorder transactions in order to extract value from other commands, commonly referred to as miner extractable value (MEV) in the cryptocurrency literature.
Ordering equality can be used to deter such side payments and ensure that the protocol orders commands fairly even though the client may be willing to pay for preferential treatment.

To use ordering equality, we must make a few assumptions.
First, denote the protocol defined fee per transaction as $f$.
This is paid by the protocol to the leader in order to ensure that a rational leader includes transactions in their block.
We also denote any client includes a fee of $f_c$ to sequence command $c$.
Finally, we denote $b_c$ as the out of band bribe paid by the client to the replicas.
In order to use our ordering equality framework, we assume that for any command, $b_c \leq \lambda$ for some constant $\lambda$.
This is the maximum willingness to pay by any client to include their transaction.
Equivalently, this protocol will only guarantee ordering equality for transactions whose bribe is at most $\lambda$.
We also require that $f_c >> \lambda$.

At this point, applying ordering equality is fairly straightforward.
The score for client $c$ is defined as $f_c$, while the noise is $b_c$.
Then, by Theorem~\ref{thm:equivalence}, we can apply the Laplace mechanism to this score in order to guarantee $\epsilon$-ordering equality.


==> long_sections/problem_long.tex <==
\section{Fair Ordering}

In order to achieve fair ordering, one must begin with identifying what fairness means.
Indeed, many notions have been trying to capture what it means that transactions are ordered in a fair manner (First-come-first-served, batch-order-fairness, and starvation-free are only a few of them). 
We follow the scheme suggested by~\cite{bercow}, where a fair ordering is one that takes into account only relevant features.
% when choosing order between requests.
% \shir{fred: partial ordering}
Among requests that share the same relevant features, equity is sought. That is, intuitively, ordering is fair if they share the same \say{chances} to be ordered one before the other.
% (a property called Ordering Equality (OE)).
Formally, they propose the $\epsilon$-Ordering Equality property, where the only relevant feature is request's invocation time.
% We now state the $\epsilon$-Ordering Equality described in~\cite{}.

We also make a slight change to the definition definition so that that relation between probabilities has a multiplicative error bound of 
$e^\epsilon$ instead of an additive error to ensure that the relative differences between probabilities are preserved. This allows for a more natural comparison across different scales, particularly when dealing with small probabilities, which would be disproportionately affected by an additive error. \shir{I was writing that based on google info, Neel does this makes sense? haha}
For completeness and simplicity, we remove the specific choosing of what is considered relevant and use different notations. We refer the reader to~\cite{bercow} for their exact definition.



\newcommand{\Io}{\mathcal{I}}
\begin{definition}[$\epsilon$-Ordering Equality]
    For any two requests $r_1,r_2$, if $r_1\sim r_2$, then $Pr[r_1\prec r_2]\leq e^{\epsilon} Pr[r_2\prec r_1]  $.

\end{definition}


% \subsection{Achieving $\epsilon$-Ordering Equality}


% In the next few sections we make a simplifying assumption. We will remove that assumption later.

% \begin{assumption}
%     Clients can precisely measure the relevant features of their request.
% \end{assumption}


In a system where clients are crash-fault, but do not experience any Byzantine behavior it seems that a fair ordering is easy to achieve.
If clients can precisely measure the relevant features of their request, record them, and attach them as metadata to the request itself. 
In turn, $\mathcal{S}$ waits for the moment the requests with the same metadata stabilize and then assigns a random order for these requests.
Unfortunately, the latter approach fails in the presence of Byzantine clients. Those clients can, among other things, send a purposely wrong set of relevant features, manipulating the output and exposing the system to vulnerabilities.
The same is true for features that can just not be measured accurately across all clients. For example, since they have different clocks.

To achieve $\epsilon$-Ordering Equality, one should be able to tell apart the noise rising from inherent system biases or Byzantine behavior. Counter-intuitively, the way in we we address the challenge of noisy information is by adding more noise. To understand how to do that, we start by reasoning about how request are perceived at $\mathcal{S}$.

To simplify, assume there is only one relevant feature for each request that is captured at $\mathcal{S}$ (as clients cannot be trusted for measurements). In practice, multiple features can be aggregated as desired.
% We dive deeper to understand what affects this measurement. It is not assigned in a void, but it is influenced not only by the requests themselves and their metadata but also by external, irrelevant information.
% To this end, w
We define the score of a request as a function
% \emph{score}$:
% $\mathcal{R}\rightarrow \mathcal{O}$
that maps a request $r$, together with both its relevant and irrelevant features to a score $score$. 
% The inputs of the function are the relevant features $\emph{metadata}$ and irrelevant features $\eta_{irr}$ associated with a specific request. 
To comply with existing deployed systems, we focus in this paper on numerical scores, where \emph{score} is computed by implicitly summing relevant and irrelevant features.
 % (e.g., time of issue+delay, block fee+bribery etc.). 


 A simple example is network delays-- a relevant piece of information is the time of invocation by the client, whereas the time frame it took the command to be sent over the network towards different replicas is irrelevant. However, unconsciously, the server sums these two values together when assigning a suggested score.
 % E.g., a client located in Brazil issues a request at $5:00$ PM. Since one of the replicas is located in India, it may receive it with a 2-minute delay, assigning $5:02$ PM as the indicator.
Note that this is not a Byzantine behavior, the server is doomed to naively make this sum, as it cannot distinguish the relevant and irrelevant information.
% Also note that in order to prevent Byzantine clients from spreading misleading information, we cannot rely on a client to provide a correct time of invocation in this example.
Another example of an additive score function is in the context of transaction fees, where the server may want to set its preferences according to the amount of revenue it makes by setting one command before the other. In this case, relevant information would be the fees corresponding to block transactions. On the other hand, any kickbacks exposed by clients are irrelevant and should be masked when aiming for fair ordering. More on that example in~\ref{sec:DP_for_miners_fees}.




Formally, 
\begin{equation*}
    \emph{score}(r)=\text{metadata}+\eta
    % \emph{score}(c)=\text{metadata}+\eta_{irr}+\eta_b
\end{equation*}
where metadata holds the relevant information and $\eta$ is the noise from irrelevant features that are implicitly biasing the score.
Our objective in this paper is to overcome inherent noise originating in the environment.


% \subsection{Achieving $\epsilon$-Ordering Equality, but not at all costs \shir{find a better name}}


Intuitively, a ``fair'' ordering mechanism should give heavy weight to the metadata component of \emph{score}, and ideally ignore the rest when assigning an order. In other words, we aim at increasing the signal of metadata and conceal $\eta$. 





As one might suspect, it is impossible to handle any amount of noise that is being added to the meaningful information when computing \emph{score}.
That is, there are cases where it is impossible to satisfy $\epsilon$-Ordering Equality. In a nutshell, when the noise in the system $\eta$ is too high, it becomes impossible to distinguish it from the metadata signal.
Therefore, we define a threshold $\lambda$ on the amount of noise we can handle. Formally, for two requests $c,c'$ we use norm L1 to reason about their difference in noise.

We make the following assumption:

\shir{clean formalization...}
\begin{assumption}
\label{assumption:bound_on_noise}
There exists a system parameter $\lambda$ s.t.
            \[\lambda =\max_{r,r'} \lVert r.\eta-r'.\eta \rVert_1 \]
where $r\sim r'$.
\end{assumption}

When a system is instantiated with the ``right'' $\lambda$, $\epsilon$-Ordering Equality can be satisfied.




% Finally, in this work we consider a \emph{fair} policy to be one that is both \emph{valid} and satisfies Ordering Equality. 

% Following the discussion from the previous section, we note that some notion of stability is inseparable from adjacent requests. I.e., relevant features must include information that can stabilize. \shir{obviously need to explain this part better}

% To be convinced, imagine that a requests relevant feature is only client id. That means that all requests coming from the same client has to be ordered in some uniform random order. This, requires a client to commit never sending anymore requests in the future, rendering a useless property for most systems.


% \shir{need to identify more carefully what is the information that is required, so I can use it later- it has to do with having an upper bound on the time until which requests with the same features can arrive}


% \subsection{Feasible Fair Policies}

% In the next few sections we make a simplifying assumption. We will remove that assumption later.

% \begin{assumption}
%     Clients can precisely measure the relevant features of their request.
% \end{assumption}


% \subsubsection{Trusted Clients}
% In a system where clients are crash-fault, but do not experience any malicious, Byzantine, behavior it seems that a fair ordering is easy to achieve.  Based on Assumption 1, clients can record the relevant features of their request and attach it as a metadata to the request itself. 
% In turn, the server waits for the moment the requests stabilize, and then assign a random order for these requests.

% \subsubsection{Byzantine Clients}

% The latter approach clearly fails in the presence of Byzantine clients. Those clients can, among other things, send a purposely wrong set of relevant features, manipulating the output order and violating the desired policy. 
% We now omit Assumption 1, as we cannot distinguish wrongly measured features from Byzantine features.

% We observe that this problem can be solved by an external tool that verifies the measure features. Indeed, our insight is that different information has different verifiability levels. Our solution will then be outsourcing the task of verifying features, or adjusting features measurement to an external abstraction (conceptually).
% \shir{I guess that if we find ourselves using DP- then DP is a way to "correct" wrongly measured features}



==> long_sections/related_work_long.tex <==


Several works have explored the concept of fairness in SMR, each proposing different approaches and properties to address biases in transaction ordering. Aequitas~\cite{} introduced two properties: receive-order-fairness and $\gamma$-batch order-fairness. The $\gamma$-batch order-fairness property ensures that if a $\gamma$ fraction of honest nodes receive a transaction $tx$ before another transaction $tx'$, then $tx$ should be ordered no later than $tx'$. The receive-order-fairness property, which would strictly enforce ordering based on when transactions are received, is deemed impossible without a strong synchrony assumption. Consequently, Aequitas focuses on implementing $\gamma$-batch order-fairness alone.

Themis~\cite{} builds on Aequitas, solving a liveness problem that arose in Aequitas' design. It provides a total ordering on transactions while respecting batch-order-fairness. However, fairness in Themis is only guaranteed at the batch level and not within individual transactions in each batch. As a result, attacks based on the specific ordering of transactions, such as front-running, remain possible. Additionally, Themis requires $4f+1$ resilience, which imposes stronger requirements than traditional SMR. Although replication itself is beyond the scope of this paper, Themis' approach is independent of the resilience model of SMR. Specifically, Bercow~\cite{} explains how SMR replicas can sample a common random variable using a secret random oracle (SRO), and while this mechanism differs from Themis, the same abstraction could be applied for arbitrary distributions.

Quick Order Fairness~\cite{} offers a property called differential order fairness, which is similar in spirit to batch-order fairness but is designed with a more efficient algorithm than Themis, providing improved complexity while maintaining similar guarantees.

Wendy~\cite{} and Pompe~\cite{} both propose the concept of fair separability, which dictates that if all honest nodes receive $tx$ before any honest node receives $tx'$, then all honest nodes should output $tx$ before $tx'$. This addresses the batch-resolution issue, providing better guarantees for transaction ordering compared to Aequitas and Themis. For $\alpha = 1$, Wendy and Pompe are very similar to $\gamma$-batch order-fairness, though they achieve better resilience thresholds. Despite this, Wendy and Pompe remain vulnerable to algorithmic biases and subtle manipulations by Byzantine clients, particularly due to their sensitivity to irrelevant transaction features, such as faster network facilities.

Bercow claims to overcome these vulnerabilities, but as analyzed in this paper, it does not fully succeed. Bercow limits its definition of relevant features to the time of issue for each transaction, which is indeed relevant for preventing specific attacks like front-running and sandwich attacks, where malicious clients try to gain profit by manipulating transaction order. However, this narrow definition fails to address scenarios where transactions have similar—but not identical—relevant features. In this work, we extend Bercow's definition to consider any type of relevant feature, introducing decaying probabilities to reorder transactions based on the differences between them. Our mechanism applies specifically to cases where irrelevant features might influence the ordering preference by adding numerical values to the relevant information. Addressing other types of noise remains an open question.

A recent work, ``Fair Ordering via Streaming Social Choice Theory''~\cite{}, strengthened the notion of batch-order fairness to $(\gamma, \delta)$-minimal-batch-order-fairness, which captures the idea that a protocol cannot distinguish between a $\delta$-fraction of faulty replicas misreporting a transaction ordering. More interestingly, this work examines fairness through the lens of social choice theory, similar to the underlying discussion in Bercow. In contrast, we examine fairness from the perspective of another computing field—databases and privacy—which we believe is more relevant and founded for addressing algorithmic bias and ensuring fairness in SMR.


==> multiple_servers.tex <==
\section{From a Single Server to Multiple Servers}

\shir{explain the problem in a low level careful way, how is it different from SMR}

Assume now that the system is composed of a set of $n$ servers, denoted $p_1,\dots,p_n$.
It is easy to implement a single server abstraction using a consensus mechanism. Indeed, agreeing on a common prefix of commands is a known and widely-researched problem: State Machine Replication (SMR). Yet, SMR on itself does not capture our policy-flavor of things, it only requires that clients commands are executed at all servers in the same order, emulating a single server.

Moreover, it is unclear what policy properties even mean in a decentralized endowment. In this context, different servers may received requests at different time, possibly in different order, rendering the set $R$ undefined, and so are the properties.
In this section, we first revise our definition and adjust them to the new model.

First, we can no longer address $t$ as the local time at server level. Instead, he time $t$ is "god's time". That could be measured, for example, as the number of steps taken in the execution by any of the participants (clients or servers). Accordingly, we denote by $R_{i,t}$ the set of requests received by server $p_i$ by time $t$. The former notation $R_t$ is now assigned with a different meaning: $R_t$ is the set of all requests received by a quorum of $f+1$ servers by time $t$\shir{maybe n-f, we'll see}. Formally,

\begin{equation*}
    R_t\defeq \{ r\ \  s.t. \ \ |\{ p_i | r\in R_{i,t}     \}| \geq f+1\}
\end{equation*}



$O_t$, in turn is the common agreed-upon sequence of requests ordered by time $t$. Similarly to SMR output, this sequence reflects a \say{synchronized} view of requests on which the set of servers have reached consensus. We denote by $O_{i,t}$ the set of requests ordered by server $p_i$ by time $t$. Ideally, for any two correct processes $p_i,p_j$ it holds that $O_{i,t}=O_{j,t}$. Reality is a bit more complicated, as some servers may be faulty. For example, servers cannot wait for all other to acknowledge some ordering of requests, because it is possible that some of them crash and will never respond, preventing any progress from taking place. Instead, the common practice it to rely on a quorum of $n-f$ servers. A natural attempt to define $O_t$ can then be:


\begin{equation*}
    O_t\defeq \{ r\ \  s.t. \ \ |\{ p_i | r\in O_{i,t}     \}| \geq n-f\}
\end{equation*}

Note that this formulation still does not imply that $O_{i,t}=O_{j,t}$ for any two correct processes $p_i,p_j$. It is possible the some servers are Byzantine and allow $p_i$ to order a request $r$, while $p_j$ may be still lagging behind at time $t$ (actually, for the current choose of $t$, even if all servers are correct there is an inherent time in which there is divergence in local views of $O_t$).
However, the intersection of quorums of size $n-f$ does imply that all local orders are a prefix of a common global order.




\shir{I'll have to make the definition more precise, as R,O of Byzantine can be whatever. would probably add *of correct servers* in the definition and change them amount to be minus f . will revise}

Given that $O_t$ is an SMR output, all the valid policy properties still hold in the new seeting with the new notations.
I sketch the proof briefly here:
\begin{itemize}
    \item Order Determinism: either we can have a valid input to be one that has f+1 signatures, or we say that a server can learn about requests from other servers as well in this case it learns bout it before ordering..
    \item Non-Blocking: from SMR liveness
    \item Consistency: 
    \item Monotonic Order:
\end{itemize}





% is pompe valid?

==> policy.tex <==
\section{Modeling Policies}

\begin{itemize}
    \item $n$ clients $c_1,\dots c_n$
    \item one server (could be implemented by multiple replicas)
    \item clients feed requests into the server
    \item server process requests in some order
\end{itemize}

The order in which requests are processes is defined by a \emph{policy}.

We're interested in the following questions: (first two are Fred's, then added more)
\begin{enumerate}
    \item What policies are feasible? What are not?
    \item What are the clients' capabilities to disrupt the enforcement of a policy?
    \item What "protections" mechanism can we offer against the latter?
    \item How do the previous answers change in the presence of Byzantine?
    
\end{enumerate}


\subsection{Specification}
Fred offered the following specification:
\begin{itemize}
    \item Initial state (denoted by $S$)
    \item Set of state transitions (This is safety = What is allowed to happen). transition is of the form $B\rightarrow S$. Where $B$ is a predicate, and $S$ is the new allowed state.
    \item Liveness = what must happen (eventually). The predicates $B$ that are eventually satisfied
\end{itemize}


A possible instantiation of a state $S$:
\begin{itemize}
    \item $CR_i$ = set of requests at client $i$
    \item $CS$ = set of requests at server
    \item $PS\subset CS$ = the set of requests that the server is going to process next
\end{itemize}
A possible instantiation of state transitions:
\begin{itemize}
                                                            
                                                            
                                                            
                                                            
       \item true $\rightarrow new r ;  CR_i=CR_i\cup\{r\}$
    \item $r\in CR_i$ $\rightarrow CR_i=CR_i\setminus\{r\} ;  CS=CS\cup\{r\}$
    \item $r\in PS$ $\rightarrow  PS=PS\setminus\{r\}$
\end{itemize}


\section{Policies desired properties}
\begin{itemize}
    \item consistency: issue time $<$ added to pending time $\leq$ execeution time (*)
    \item execution time does not change once assigned (*)
    \item policy only depends on the current pending set (*)
    \item wellformness of requests : assumption on request format (*)
    \item non blocking: if pending is not empty, policy must output (!)
    \item there's a bound on the maximal requests that the policy can output at a time (due to limited resources) (*)
    \item a client cannot cancel a request (or can he? this might be desirable but not feasible in asynchrony) (*)
    
    \item integrity: every request in the pool was previously sen by a client (*)
    \item starvation free = every request eventually gets into the pool, and eventually executed (!, implies 5)
\end{itemize}

question; are there infeasible policies that satisfy those properties?




==> problem_old.tex <==

    
\section{The Ordering Problem}
% \subsection{The Ordering Problem}

In the ordering problem, a server decides on the total order of the input requests received by clients, subject to some \emph{policy} $\mathcal{P}$. This order is the one by which requests are processed.
This problem is far from being new, but we believe the theoretical foundation around it is lacking. A similar field, for example, is queue theory, where the focus is load balancing and performance metrics. Instead, we aim to lay grounds to study the feasibility of different ordering methods.

We formalize this task using notions of requests, the target policy, and an output schedule. 
Intuitively speaking, the server produces an output schedule that aims to follow a \emph{policy} $\mathcal{P}$ when choosing an order for the requests.
Formally, the set $R$ contains requests. 
The \emph{policy} $\mathcal{P}$ is a predicate that applies to a pair of requests such that $\mathcal{P}(r_1,r_2)$ is satisfied if and only if $r_1$ must appear before $r_2$ in the output schedule.
$\mathcal{P}$ projects a strict partial order $\prec$ on the set of requests $R$.
This partial order encapsulates the desired order on requests, that a solution to the ordering problem must preserve.
Finally, a \emph{schedule} $\prec_{total}$ is a total order on $R$.
Formally,
\begin{definition}[Ordering] Algorithm $\mathcal{A}$ solves the ordering problem if, given $R$ and $\prec$, it produces output sequence $\prec_{total}$ such that for any two requests $r_1,r_2\in R$ it holds that $r_1\prec r_2 \Rightarrow r_1\prec_{total} r_2$.
    
\end{definition}

 
 Or: $\mathcal{P}(r_1, r_2)=\textit{true}\Rightarrow r_1\prec_{total} r_2$.

$\mathcal{A}$ is an online algorithm; requests are not known in advance but are fed into the algorithm with time.
Although it seems an empty statement to check whether a policy is satisfied with a single server following the prescribed partial order. We will see that some policies are either infeasible to implement or useless.



\paragraph{Notations.}
% We use the notion of \emph{pending set} to capture
As we assume a single server, we can rely on the notion of time, as captured locally at that server.
We use the notation $R_t\subset R$ to capture the set of requests received by the server up to and including time $t$. I.e., requests that were delivered by the underlying communication protocol.
Similarly, we use $O_t$ as the subset of $\prec_{total}$ that was determined by time $t$, by the algorithm $\mathcal{A}$. We also refer to $O_t$ as the lineage of requests within the set, according to their well-defined order.
As a result, $P_t=O_t\setminus R_t$ reflects the pending set at time $t$. These are requests that were received but were not yet ordered. 



\subsection{Meaningful Policies}







% We now explore different properties to understand which policies are desirable and which are feasible.
To fulfill meaningful properties on ordering output, we start by painting general properties, which we require all ordering outputs to satisfy. These properties can hint at which policies are desirable and feasible.


The first property, \emph{Order Determinism}, requires that an order only depends on previously received requests $R$. I.e., a request cannot be ordered before the server learns about it.
% That is, it is impossible to condition one request's order on an input request that has not been delivered yet.
% It is easy to see that any policy that does not satisfy Order Determinism is infeasible in an asynchronous system, where undelivered requests are in the bivalent state of being delivered in the future, or get lost in space. \shir{can be proven formally}.
% Formally, an output schedule satisfies Order Determinism if the following holds:

\begin{definition}[Order Determinism]
The order $O_t$ at time $t$ should be a function of the set of requests $R_t$ received up to that point. 
\end{definition}



Next, we introduce a liveness property called \emph{Non-Blocking}.
This property states that if any requests were received but were not assigned an order, the server must eventually produce an order that includes these requests. This property prevents the server from being idle forever or deadlocked when there are pending tasks. 
%Our model assumes every request sent by a client is eventually delivered to the server and added to the pending set.
Formally,

% \begin{definition}[Non-Blocking]
% If there are any pending requests at time $t$, the policy must produce an output order $O_t$. I.e., $P_t\neq \varnothing \implies O_t\neq \varnothing$.
% \end{definition}

% Another option: where you can wait to see more inputs
\begin{definition}[Non-Blocking]
If there are any pending requests at time $t_1$, the policy must eventually produce an output order $O_{t_2}$ that includes them, for some $t_2>t_1$. I.e., $P_{t_1}\neq \varnothing \implies P_{t_1}\subset O_{t_2}$.
\end{definition}
\shir{ maybe should be $\cap$ and not $\subset$, so that it's ok to starve some...}

Finally, the following two properties assure that the order is consistent over time, both in the presence of new requests (\emph{Monotonic Order}) and their absence (\emph{Consistency)}. Intuitively, this means that the existing output order cannot be manipulated with time.

\begin{definition}[Consistency]
If no new requests are received between $t_1$ and $t_2$, then the order at $t_2$ is consistent with the order at $t_1$. I.e., $R_{t_1}=R_{t_2}\implies O_{t_1}=O_{t_2}$
\end{definition}


\begin{definition}[Monotonic Order]
If a new request $r$ is received at time $t_2$ s.t. $R_{t_2}=R_{t_1}\cup\{r\}$, then the order $O_{t_2}$ is be a valid extension of the order $O_{t_1}$.
\end{definition}

\paragraph{to policies:}
The four properties above are what make a \emph{valid} order.
However, it may be the case that the only way to solve the ordering problem for some policies P is by violating one of those properties. 

Note that the two trivial predicates are either always solvable (the empty relation) or always not solvable (the universal one). We'll also say that a policy is trivial if all comparable requests are pair-originated at the same client. We claim this is trivial as in this case the ordering problem can already be solved on the client level.

\begin{theorem}
It is impossible to solve the valid ordering problem in asynchrony for arbitrary non-trivial policy $\mathcal{P}$.
\end{theorem}
\begin{proof}

Assume by way of contradiction that there exists algorithm $\mathcal{A}$ that solves the valid ordering problem in asynchrony. Let $P$ be a policy, and $r_1,r_2$ a pair such that $P(r_1,r_2)=true$. such a pair exists since the policy is not trivial. Let $\pi$ be an execution in which both $r_1$ and $r_2$ are sent by clients $c_1, c_2$, resp.


Let $\sigma_{r_2}$ be an execution where, out of all clients, only $c_2$ takes steps by sending $r_2$ to the server, and $t$ is the time $\mathcal{S}$ receives $r_2$.
By Non-Blocking, there must be a time $t<t'$ such that $r_2$ is output by $\mathcal{S}$ by time $t'$.
Now consider a second execution $\sigma_{both}$ in which both $c_1$ and $c_2$ take steps, by sending $r_1,r_2$ to $\mathcal{S}$, resp.
As before, $t$ is the time $\mathcal{S}$ receives $r_2$ and $r_1$ is received at $t'+1$.
Due to asynchrony, $\sigma_{r_2}$ and $\sigma_{both}$ are indistinguishable to $\mathcal{S}$ up until time $t'+1$. Therefore, in 
$\sigma_{both}$ $r_2$ is output by $\mathcal{S}$ at $t'$.
Further, by Non-Blocking, there must be a time $t'+1<t''$ such that $r_1$ is output by $\mathcal{S}$ by time $t''$.
In both executions, by Order Determinism, $O_{t'}$ contains $r_2$ and $r_2$ only.
Therefore, in $\sigma_{both}$, by Monotonic Order, $r_1$ must be lineaged after $r_2$, violating $\mathcal{P}$
% In both executions, by Order Determinism, $O_{t'}$ contains $r_2$ and $r_2$ only and remains that way until $t'+1$ (consistency). 


% To comply with order determinism it must be that p is not time-dependent... otherwise for $r1<r2$ we delay r1 until r2 is output (by nonblocking).
\end{proof}


To circumvent this impossibility result, we next draw a required restriction on policies so that the output order can be valid in any environment.
% Policies that follow these restrictions are called valid policies.






Following~\cite{SMR-tutorial of fred} we propose the notion of stable policy. A stable policy can guarantee some notion of "stability" in the environment in which it applies. Intuitively, stability means that if r1<r2 there must be a moment in which I know preferred requests cannot arrive.
A policy is stable if all requests on which it is defined are guaranteed to become stable, according to ~\cite{tutorial} notion.

$r$ is stable at time $t$ if $\forall r'$ such that $r'<r$, $r'$ will not be delivered at $S$ in the execution.

\begin{definition}[stability]
A Policy $P$ satisfies stability if for any two requests $r_1,r_2$ it holds that $P(r1,r2)=true\implies \exists t $ known to $\mathcal{S}$ s.t. if $r_1$ is not delivered by $t$ it will not be delivered at all.
\end{definition}


Note that stability is necessary but not sufficient. While there may be a moment in which both r1 and r2 are stable, for example, clients stop sending requests at X. It is still required to be able to tell which of the stable requests should come first. To this end, we require that a policy is computable. Given that two requests, have arrived- we must be able to compute P if defined for the pair. If P is not defined then the output schedule makes no difference and we can output in whatever order.

All in all, we want there to be a moment in time where we can say - it is safe to order R now. because I know all preceding requests that may arrive have arrived, and I've already ordered them. 




We say that a policy that satisfies those restrictions is a \emph{valid} policy.

% In addition, we define a policy to be \emph{feasible}, if there is an algorithm that the server can run to enforce that policy. That is, no matter what requests are sent as input by the clients, the outcome trace of the execution following the algorithm is according to the policy.

\shir{Although the impossibility is defined for synchrony, I'm not sure it's possible in synchrony as well.
If a policy is time-dependent, then synchrony may help.}



\shir{maybe put this example somewhere}
As a first example, let us consider the first-come-first-served policy (FCFS). Following this policy, a server that receives a request immediately orders it after all previously received requests. The reader can verify that FCFS is a valid and feasible policy. Indeed, FCFS is a favorable method for ordering requests in many deployed systems~\cite{add citations}. 

% However, we note that \emph{valid} and \emph{feasible} are not tied together. For example, a policy in which the server does not order any request is feasible but clearly not valid.
% On the contrary, a policy that order requests according to information that is not extricable by the server may be a valid one, as it does not violate any property, but is infeasible to implement. An example for such policy could be one that agree with FCFS, but break ties according to the clients' lucky number (assuming it is unpredictable and not provided with the request).



\section{Fair Policies and the surprising connection to DP}




% So far we discussed pairs of requests that has relative order defined.

Considering real-life systems, a valid policy is necessary\shir{With the exception that the properties can be adjusted to not the receipt of requests, but just knowing of requests-that's how ziplog works} but is often not sufficient. Taking into account factors such as different clients hardware~\cite{}, possible attacks~\cite{} and legal requirements~\cite{}, more and more system designers are also require some notion of fairness in the output order. 
Indeed, there is a growing line of works on the subject of fair ordering, with different application-specific properties~\cite{}. Notably, a recent work aims to capture the general concept of fair ordering~\cite{pompe 2}. They present the principle of \emph{impartiality}, captured in the $\epsilon$-Ordering Equality property. The idea behind it is that a requests is composed of different features, some of them are \emph{relevant} for ordering, while other are \emph{irrelevant}. A fair ordering suggests that orders with the exact same relevant features has almost identical probabilities to be ordered one before the other (up to some small parameter $\epsilon$).



% ----


% \subsection{model extention}


% \shir{this entire part can be later when talking about fairness}
\paragraph{Model Extention.} 
A request $r$ issued by a client is represented as a finite vector, in which each entry is a different feature. I.e., $r=\langle f_1,f_2,\dots f_k \rangle$. These features can include information originated by the client who issued them, network information, and/or information recorded at the server when they arrived. 
For example, possible features are client id, type of request, time of arrival at $\mathcal{S}$ etc.
We use that notation $r[i]$ to address $r$'s $i^{th}$ feature.
Following~\cite{pompe2}, we divide features into two categories of relevant and irrelevant features. As the name suggests, there is a partition of each request into the two distinct sets. Unlike~\cite{pompe2}, we leave it to the system designer to specify the desired partition.

% We assume a single feature is comparable among other requests.
% That is, we can tell the result of predicates of the form $r_1[i] <? r_2[i]$, for two different requests $r_1, r_2$.
% We do not require in this work that requests are comparable, but we do think this could be an interesting to do in the future.
% For example, for two requests $r_1$ and $r_2$ that has 2 features if $r_1[1] < r_2[1]$ and $r_1[2] > r_2[2]$, it is not defined whether $r_1>r_2$ or $r_1<r_2$.
Whereas the policy $\mathcal{P}$ may not be defined for all pairs of requests, we do claim that it is possible to say that $r_1=r_2$, if the two requests \say{agree} on all indexes.
More specific and useful in our work, we are interested in the relation between requests based on their relevant features.
We say that $r_1$ and $r_2$ are \emph{adjacent}, denoted as $r_1 \sim r_2$, if and only if their relevant features are the same, with respect to a fixed partition of the features.

% ----

% As a study case, they describe an example where the relevant feature is the time each client issues a request. In this scenario, an ordering mechanism that gives higher priority to clients with better network connectivity is considered unfair.


\paragraph{}


On a high-level, a policy $\mathcal{P}$ determines the order according to some \say{before} notion, while fairness determines what should happen if the equal predicate applies.

When defining the fairness property, Pompe2 falls short of their attempt to generalize, and instantiate it only for a relevant feature that is the invocation time at the client (from god's perspective). We imagine that different systems can decide to optimize for other selection of relevant features. We now state the $\epsilon$-Ordering Equality described in~\cite{}. For completeness and simplicity, we remove the specific choosing of what is considered relevant, and use different notations. We refer the reader to~\cite{} for their exact definition.


\newcommand{\Io}{\mathcal{I}}
\begin{definition}[$\epsilon$-Ordering Equality]
    For any two requests $r_1,r_2$, if $r_1\sim r_2$, then $|Pr[r_1\prec r_2]-Pr[r_2\prec r_1]| \leq \epsilon$.

\end{definition}

\shir{we might go back and modify further, choosing the multiplicative error factor, as in the DP writing}



Finally, in this work we consider a \emph{fair} policy to be one that is both \emph{valid} and satisfies Ordering Equality. 

Following the discussion from the previous section, we note that some notion of stability is inseparable from adjacent requests. I.e., relevant features must include information that can stabilize. \shir{obviously need to explain this part better}

To be convinced, imagine that a requests relevant feature is only client id. That means that all requests coming from the same client has to be ordered in some uniform random order. This, requires a client to commit never sending anymore requests in the future, rendering a useless property for most systems.


% \shir{need to identify more carefully what is the information that is required, so I can use it later- it has to do with having an upper bound on the time until which requests with the same features can arrive}


\subsection{Feasible Fair Policies}

In the next few sections we make a simplifying assumption. We will remove that assumption later.

\begin{assumption}
    Clients can precisely measure the relevant features of their request.
\end{assumption}


\subsubsection{Trusted Clients}
In a system where clients are crash-fault, but do not experience any malicious, Byzantine, behavior it seems that a fair ordering is easy to achieve.  Based on Assumption 1, clients can record the relevant features of their request and attach it as a metadata to the request itself. 
In turn, the server waits for the moment the requests stabilize, and then assign a random order for these requests.

\subsubsection{Byzantine Clients}

The latter approach clearly fails in the presence of Byzantine clients. Those clients can, among other things, send a purposely wrong set of relevant features, manipulating the output order and violating the desired policy. 
We now omit Assumption 1, as we cannot distinguish wrongly measured features from Byzantine features.

% We observe that this problem can be solved by an external tool that verifies the measure features. Indeed, our insight is that different information has different verifiability levels. Our solution will then be outsourcing the task of verifying features, or adjusting features measurement to an external abstraction (conceptually).
% \shir{I guess that if we find ourselves using DP- then DP is a way to "correct" wrongly measured features}

\section{NEW}
The problem is now how to approximate policies in the case they are not commutable in a precise manner.
The solution is noise.


==> write_up.tex <==
\section{Write-Up}

% \begin{enumerate}
%     \item assume everyone is trusted
%     \item  time is inherent
%     \item byzantine clients, trusted servers
%     \item different 'information' has different verifability levels
%     \item private-> verify with external entity
% \end{enumerate}



% \shir{parital order of requests: requets are vectors}
% \shir{aximoms fo a good polsicy}
% set theory definition of a policy-partial order, schedule=total order, when is a schedule satisfy policy.?
% point out in online system, requests periodically increase set of requests and decrresaing the scheulde online 




%fairness notions
This paper seeks to navigate the field of \emph{fair} ordering of commands.
Fairness is a broad and subjective term, and many notions have been trying to capture what it means that transactions are ordered in a fair manner (FCFS, round robin, and starvation-free are only a few of them).
We follow the scheme suggested by~\cite{pompe2}, where every request has a set of features associated with it. Some of those features are considered to be \emph{relevant} and some are \emph{irrelevant}.
A fair ordering is then an ordering that takes into account only relevant features.
% \shir{fred: partial ordering}
Among requests that share the same relevant features, equity is sought. That is, ordering is fair if they share the same \say{chances} to be ordered one before the other (a property called Ordering Equality(OE)).
Note that the specific features that are relevant and irrelevant are not captured in the definition, and in fact, most of the existing fairness properties can be considered to satisfy OE, when instantiated with the \say{right} choice of relevant features.

For example, FCFS is equivalent to equal opportunity if the relevant feature is the time of arrival at the system. We note that it is sufficient to define relevant features, and then the irrelevant feature is the complementary information of that request.
% Round robin also satisfies OE, if the relevant feature is "the number of the requests issued by a single client" (that is true, up to the order in which the round robins go, to be precise that would be true if at any "round" a random permutation of the clients is picked).
% starvation-free is not captured by OE.


% policy formulation

Equipped with a concrete fairness definition in hand, we aim to systematically study and answer the question:

\begin{center}
\textit{
Under what \textbf{conditions} can one achieve \textbf{fair} ordering?
}
\end{center}

Note that there is an inherent degree of freedom to that question: the variables are the system condition/model and the relevant features being examined. By fixing one of them, we can solve the other.

Our starting point is even more fundamental. We wish to know what properties any ordering policy can and should satisfy, fairness is just an example of such.

Distributed systems are often examined under the lens of \emph{executions}, which elegantly captures different nodes' actions, be it by looking at their internal states, or exchanged messages (could also be via shared memory). Those executions have been studied for decades, and there are many common properties that one may want to prove about their distributed system. Avoiding deadlock and being fault-tolerant are desired, to name a few.
This study is so extensive, that those properties are further classified into families of properties: such as safety and liveness. Various other such "families" exist, although it is proved by Fred that any property lies somewhere in the intersection of these two.

We start by narrowing the discussion to not just any distributed task, but the task of ordering requests. We hope this smaller scope will allow us to more carefully research that problem and obtain new insights, specific to that problem.


We start by proposing a new framework that captures the concept of ordering.
